SPADE: A Spectral Method for Black-Box Adversarial Robustness Evaluation

A black-box spectral method is introduced for evaluating the adversarial robustness of a given machine learning (ML) model. Our approach, named SPADE, exploits bijective distance mapping between the input/output graphs constructed for approximating the manifolds corresponding to the input/output data. By leveraging the generalized Courant-Fischer theorem, we propose a SPADE score for evaluating the adversarial robustness of a given model, which is proved to be an upper bound of the best Lipschitz constant under the manifold setting. To reveal the most non-robust data samples highly vulnerable to adversarial attacks, we develop a spectral graph embedding procedure leveraging dominant generalized eigenvectors. This embedding step allows assigning each data sample a robustness score that can be further harnessed for more effective adversarial training. Our experiments show the proposed SPADE method leads to promising empirical results for neural network models that are adversarially trained with the MNIST and CIFAR-10 data sets.

==> table/cifar_adv_normal.tex <==
\begin{table*}[ht!]
\caption{Model SPADE scores variation between CIFAR-10 standard test set and CIFAR-10 adversarial test set .}
\label{cifar_adv_normal}
%\vskip 0.15in
\vspace{0pt}
\begin{center}
\begin{small}
\small
\begin{sc}
\begin{tabular}{lccccc}
\toprule
Networks & $\epsilon = 0$ & $\epsilon = 0.25$ & $\epsilon = 0.5$ & $\epsilon = 1$ \\
\midrule
SPADE score of adversarial sample ($\epsilon = 0.25$, 20NN)      & $288.22$ & $182.82$ & $158.20$ & $159.67$ \\
SPADE score of standard sample ($\epsilon = 0$, 20NN)   & $353.04$ & $203.32$ & $165.78$ & $134.90$ \\

\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
%\vskip -0.1in
\vspace{-15pt}
\end{table*}

==> table/notation.tex <==
\begin{table}
%\scalebox{1.29}
\centering \caption{Symbols and their denotations in this work}
\vspace{5pt}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{ |c|c|c|c| }
%  \multicolumn{4}{|c|}{Symbols and Denotations Used in This Work} \\
 \hline
 Symbol& Denotation &Symbol& Denotation\\
 \hline
 $X\in {\mathbb{R} ^{M\times N}}$&  Input data & $Y\in {\mathbb{R} ^{D\times N}}$& Output data\\
 $G_X = (V, E_{X})$   & Input graph & $G_Y = (V, E_{Y})$   & Output graph\\    $\mathbf{L_{X}}\in {\mathbb{R} ^{N\times N}}$& Laplacian of  $G_X$ 
& $\mathbf{L_{Y}}\in {\mathbb{R} ^{N\times N}}$  & Laplacian of  $G_Y$\\
   $d_X\in {\mathbb{R^+}}$& Distance in  $G_X$ 
& $d_Y\in {\mathbb{R^+}}$& Distance in    $G_Y$\\
$\gamma^F$ & Dist. map. dist.&$\zeta^F$ & Cut map. dist.\\
$\sigma$ & Lap. eigenvalue&$u\in {\mathbb{R} ^{N}}$ & Lap. eigenvector\\
$\lambda$ & Gen. eigenvalue&$v\in {\mathbb{R} ^{N}}$ & Gen. eigenvector\\
 \hline
 \end{tabular}\label{table:symbol}
 }
\end{table}
